LLAMA: Stellar populations in the nuclei of ultra hard X-ray selected AGN and matched inactive galaxies

The relation between nuclear ($\lesssim$ 50 pc) star formation and nuclear galactic activity is still elusive: theoretical models predict a link between the two, but it is unclear whether active galactic nuclei (AGNs) should appear at the same time, before or after nuclear star formation activity is ongoing. We present a study of this relation in a complete, volume-limited sample of nine of the most luminous ($\log L_{\rm 14-195 keV} > 10^{42.5}$ erg/s) local AGNs (the LLAMA sample), including a sample of 18 inactive control galaxies (6 star-forming; 12 passive) that are matched by Hubble type, stellar mass (9.5 $\lesssim$ log M_star/M_sun $\lesssim$ 10.5), inclination and distance. This allows us to calibrate our methods on the control sample and perform a differential analysis between the AGN and control samples. We perform stellar population synthesis on VLT/X-SHOOTER spectra in an aperture corresponding to a physical radius of $\approx$ 150 pc. We find young ($\lesssim$ 30 Myr) stellar populations in seven out of nine AGNs and in four out of six star-forming control galaxies. In the non-star-forming control population, in contrast, only two out of twelve galaxies show such a population. We further show that these young populations are not indicative of ongoing star-formation, providing evidence for models that see AGN activity as a consequence of nuclear star formation. Based on the similar nuclear star-formation histories of AGNs and star-forming control galaxies, we speculate that the latter may turn into the former for some fraction of their time. Under this assumption, and making use of the volume-completeness of our sample, we infer that the AGN phase lasts for about 5 % of the nuclear starburst phase.

==> journals.tex <==
%%
%% aastex.cls journal abbreviations
%%
\newcommand{\jnlref}[1]{{ \textsf #1}}
\newcommand\aj{\jnlref{AJ}}%
          % Astronomical Journal
\newcommand\actaa{\jnlref{Acta Astron.}}%
  % Acta Astronomica
\newcommand\araa{\jnlref{ARA\&A}}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{\jnlref{ApJ}}%
          % Astrophysical Journal
\newcommand\apjl{\jnlref{ApJ}}%
          % Astrophysical Journal, Letters
\newcommand\apjs{\jnlref{ApJS}}%
          % Astrophysical Journal, Supplement
\newcommand\ao{\jnlref{Appl.~Opt.}}%
          % Applied Optics
\newcommand\apss{\jnlref{Ap\&SS}}%
          % Astrophysics and Space Science
\newcommand\aap{\jnlref{A\&A}}%
          % Astronomy and Astrophysics
\newcommand\aapr{\jnlref{A\&A~Rev.}}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{\jnlref{A\&AS}}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{\jnlref{AZh}}%
          % Astronomicheskii Zhurnal
\newcommand\baas{\jnlref{BAAS}}%
          % Bulletin of the AAS
\newcommand\caa{\jnlref{Chinese Astron. Astrophys.}}%
  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{\jnlref{Chinese J. Astron. Astrophys.}}%
  % Chinese Journal of Astronomy and Astrophysics
\newcommand\icarus{\jnlref{Icarus}}%
  % Icarus
\newcommand\jcap{\jnlref{J. Cosmology Astropart. Phys.}}%
  % Journal of Cosmology and Astroparticle Physics
\newcommand\jrasc{\jnlref{JRASC}}%
          % Journal of the RAS of Canada
\newcommand\memras{\jnlref{MmRAS}}%
          % Memoirs of the RAS
\newcommand\mnras{\jnlref{MNRAS}}%
          % Monthly Notices of the RAS
\newcommand\na{\jnlref{New A}}%
  % New Astronomy
\newcommand\nar{\jnlref{New A Rev.}}%
  % New Astronomy Review
\newcommand\pra{\jnlref{Phys.~Rev.~A}}%
          % Physical Review A: General Physics
\newcommand\prb{\jnlref{Phys.~Rev.~B}}%
          % Physical Review B: Solid State
\newcommand\prc{\jnlref{Phys.~Rev.~C}}%
          % Physical Review C
\newcommand\prd{\jnlref{Phys.~Rev.~D}}%
          % Physical Review D
\newcommand\pre{\jnlref{Phys.~Rev.~E}}%
          % Physical Review E
\newcommand\prl{\jnlref{Phys.~Rev.~Lett.}}%
          % Physical Review Letters
\newcommand\pasa{\jnlref{PASA}}%
  % Publications of the Astron. Soc. of Australia
\newcommand\pasp{\jnlref{PASP}}%
          % Publications of the ASP
\newcommand\pasj{\jnlref{PASJ}}%
          % Publications of the ASJ
\newcommand\qjras{\jnlref{QJRAS}}%
          % Quarterly Journal of the RAS
\newcommand\rmxaa{\jnlref{Rev. Mexicana Astron. Astrofis.}}%
  % Revista Mexicana de Astronomia y Astrofisica
\newcommand\skytel{\jnlref{S\&T}}%
          % Sky and Telescope
\newcommand\solphys{\jnlref{Sol.~Phys.}}%
          % Solar Physics
\newcommand\sovast{\jnlref{Soviet~Ast.}}%
          % Soviet Astronomy
\newcommand\ssr{\jnlref{Space~Sci.~Rev.}}%
          % Space Science Reviews
\newcommand\zap{\jnlref{ZAp}}%
          % Zeitschrift fuer Astrophysik
\newcommand\nat{\jnlref{Nature}}%
          % Nature
\newcommand\iaucirc{\jnlref{IAU~Circ.}}%
          % IAU Cirulars
\newcommand\aplett{\jnlref{Astrophys.~Lett.}}%
          % Astrophysics Letters and Communications
\newcommand\apspr{\jnlref{Astrophys.~Space~Phys.~Res.}}%
          % Astrophysics Space Physics Research
\newcommand\bain{\jnlref{Bull.~Astron.~Inst.~Netherlands}}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{\jnlref{Fund.~Cosmic~Phys.}}%
          % Fundamental Cosmic Physics
\newcommand\gca{\jnlref{Geochim.~Cosmochim.~Acta}}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{\jnlref{Geophys.~Res.~Lett.}}%
          % Geophysics Research Letters
\newcommand\jcp{\jnlref{J.~Chem.~Phys.}}%
          % Journal of Chemical Physics
\newcommand\jgr{\jnlref{J.~Geophys.~Res.}}%
          % Journal of Geophysical Research
\newcommand\jqsrt{\jnlref{J.~Quant.~Spec.~Radiat.~Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{\jnlref{Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{\jnlref{Nucl.~Phys.~A}}%
          % Nuclear Physics A
\newcommand\physrep{\jnlref{Phys.~Rep.}}%
          % Physics Reports
\newcommand\physscr{\jnlref{Phys.~Scr}}%
          % Physica Scripta
\newcommand\planss{\jnlref{Planet.~Space~Sci.}}%
          % Planetary Space Science
\newcommand\procspie{\jnlref{Proc.~SPIE}}%
          % Proceedings of the SPIE
